Leak, Cheat, Repeat: Data Contamination and Evaluation Malpractices in Closed-Source LLMs

Natural Language Processing (NLP) research is increasingly focusing on the use of Large Language Models (LLMs), with some of the most popular ones being either fully or partially closed-source. The lack of access to model details, especially regarding training data, has repeatedly raised concerns about data contamination among researchers. Several attempts have been made to address this issue, but they are limited to anecdotal evidence and trial and error. Additionally, they overlook the problem of \emph{indirect} data leaking, where models are iteratively improved by using data coming from users. In this work, we conduct the first systematic analysis of work using OpenAI's GPT-3.5 and GPT-4, the most prominently used LLMs today, in the context of data contamination. By analysing 255 papers and considering OpenAI's data usage policy, we extensively document the amount of data leaked to these models during the first year after the model's release. We report that these models have been globally exposed to $\sim$4.7M samples from 263 benchmarks. At the same time, we document a number of evaluation malpractices emerging in the reviewed papers, such as unfair or missing baseline comparisons and reproducibility issues. We release our results as a collaborative project on https://leak-llm.github.io/, where other researchers can contribute to our efforts.

==> review.tex <==
\begin{itemize} 
 \item LLM-contamination~\cite{paper0}
\item Time Travel in LLMs: Tracing Data Contamination in Large Language Models~\cite{golchin2023time}
\item Don't Stop Pretraining: Adapt Language Models to Domains and Tasks~\cite{gururangan-etal-2020-dont}
\item Can we trust the evaluation on ChatGPT?~\cite{paper3}
\item How Close is ChatGPT to Human Experts? Comparison Corpus, Evaluation, and Detection~\cite{paper4}
\item GPTEval: A Survey on Assessments of ChatGPT and GPT-4~\cite{paper5}
\item A Systematic Study and Comprehensive Evaluation of ChatGPT on Benchmark Datasets~\cite{paper6}
\item Quantifying Memorization Across Neural Language Models~\cite{paper7}
\item Preventing Generation of Verbatim Memorization in Language Models Gives a False Sense of Privacy~\cite{ippolito-etal-2023-preventing}
\item List of various ChatGPT evaluations~\cite{paper9}
\item GPT-4 Technical Report~\cite{paper10}
\item Zeno Chatbot Report~\cite{paper11}
\item A Multitask, Multilingual, Multimodal Evaluation of ChatGPT on Reasoning, Hallucination, and Interactivity~\cite{paper12}
\item Don’t Stop Pretraining? Make Promp-based Fine-tuning Powerful Learner~\cite{shi2023dont}
\item How Good Are GPT Models at Machine Translation? A Comprehensive Evaluation~\cite{paper14}
\item Is ChatGPT A Good Translator? Yes With GPT-4 As The Engine~\cite{paper15}
\item Is Chatgpt A General-purpose Natural Language Processing Task Solver?~\cite{paper16}
\item Extractive summarization via ChatGPT for faithful summary generation~\cite{paper17}
\item Chatgpt or grammarly? evaluating chatgpt on grammatical error correction benchmark~\cite{paper18}
\item Will affective computing emerge from foundation models and general ai? A first evaluation on chatgpt~\cite{paper19}
\item ChatGPT: Jack of all trades, master of none~\cite{chatpgt-jack-trades-master-none}
\item Zero-Shot Information Extraction via Chatting with ChatGPT~\cite{paper21}
\item Is ChatGPT Good at Search? Investigating Large Language Models as Re-Ranking Agent~\cite{paper22}
\item Is ChatGPT a Good NLG Evaluator? A Preliminary Study~\cite{paper23}
\item G-EVAL: NLG Evaluation using GPT-4 with Better Human Alignment~\cite{paper24}
\item Large Language Models Are State-of-the-Art Evaluators of Translation Quality~\cite{paper25}
\item ChatGPT Outperforms Crowd-workers For Text-annotation Tasks~\cite{paper26}
\item SuperCLUE: A Comprehensive Chinese Large Language Model Benchmark~\cite{paper27}
\item C-eval: A multi-level multi-discipline chinese evaluation suite for foundation models~\cite{paper28}
\item ChatGPT beyond English: Towards a comprehensive evaluation of large language models in multilingual learning~\cite{paper29}
\item Zero-Shot Cross-Lingual Summarization via Large Language Models~\cite{paper30}
\item A categorical archive of chatgpt failures~\cite{paper31}
\item Benchmarks for automated commonsense reasoning: A survey~\cite{paper32}
\item Is ChatGPT a Good Causal Reasoner? A Comprehensive Evaluation.~\cite{paper33}
\item Causal reasoning and large language models: Opening a new frontier for causality~\cite{paper34}
\item Theory of mind may have spontaneously emerged in large language models~\cite{paper35}
\item Boosting Theory-of-Mind Performance in Large Language Models via Prompting~\cite{paper36}
\item Does ChatGPT have Theory of Mind?~\cite{paper37}
\item Can ChatGPT Defend the Truth? Automatic Dialectical Evaluation Elicits LLMs' Deficiencies in Reasoning~\cite{paper38}
\item Evaluating the logical reasoning ability of chatgpt and gpt-4~\cite{paper39}
\item We're Afraid Language Models Aren't Modeling Ambiguity~\cite{paper40}
\item Sparks of artificial general intelligence: Early experiments with gpt-4~\cite{paper41}
\item Chatgpt participates in a computer science exam~\cite{paper42}
\item Can llm already serve as a database interface? a big bench for large-scale database grounded text-to-sqls~\cite{paper43}
\item Mathematical capabilities of chatgpt~\cite{paper44}
\item Could an artificial-intelligence agent pass an introductory physics course?~\cite{paper45}
\item Investigating the Use of an Artificial Intelligence Chatbot with General Chemistry Exam Questions~\cite{paper46}
\item How do physics students evaluate artificial intelligence responses on comprehension questions? A study on the perceived scientific accuracy and linguistic quality of ChatGPT~\cite{paper47}
\item Chatgpt goes to law school~\cite{paper48}
\item ChatGPT has aced the test of understanding in college economics: Now what?~\cite{paper49}
\item The Wall Street Neophyte: A Zero-Shot Analysis of ChatGPT Over MultiModal Stock Movement Prediction Challenges~\cite{paper50}
\item How Does ChatGPT Perform on the United States Medical Licensing Examination? The Implications of Large Language Models for Medical Education and Knowledge Assessment~\cite{paper51}
\item Performance of ChatGPT on USMLE: Potential for AI-assisted medical education using large language models~\cite{paper52}
\item Evaluating the performance of chatgpt in ophthalmology: An analysis of its successes and shortcomings~\cite{paper53}
\item Diagnostic Accuracy of Differential-Diagnosis Lists Generated by Generative Pretrained Transformer 3 Chatbot for Clinical Vignettes with Common Chief Complaints: A Pilot Study~\cite{paper54}
\item Assessing the utility of ChatGPT throughout the entire clinical workflow~\cite{paper55}
\item ChatGPT as a medical doctor? A diagnostic accuracy study on common and rare diseases~\cite{paper56}
\item Can AI tell good stories? narrative transportation and persuasion with ChatGPT~\cite{paper57}
\item Benchmarking Foundation Models with Language-Model-as-an-Examiner~\cite{paper58}
\item Chatgpt: A meta-analysis after 2.5 months~\cite{paper59}
\item Causal-discovery performance of chatgpt in the context of neuropathic pain diagnosis~\cite{paper60}
\item Summary of ChatGPT-Related Research and Perspective Towards the Future of Large Language Models~\cite{paper61}
\item Harnessing the power of llms in practice: A survey on chatgpt and beyond~\cite{paper62}
\item Holistic evaluation of language models~\cite{paper63}
\item A Survey on Evaluation of Large Language Models~\cite{paper64}
\item Can chatgpt understand too? a comparative study on chatgpt and fine-tuned bert~\cite{paper65}
\item On the robustness of chatgpt: An adversarial and out-of-distribution perspective~\cite{paper66}
\item An Independent Evaluation of ChatGPT on Mathematical Word Problems (MWP)~\cite{paper67}
\item Can ChatGPT Replace Traditional KBQA Models? An In-depth Analysis of the Question Answering Performance of the GPT LLM Family~\cite{paper68}
\item Instruction tuning with gpt-4~\cite{paper69}
\item How Robust is GPT-3.5 to Predecessors? A Comprehensive Study on Language Understanding Tasks~\cite{paper70}
\item Consistency analysis of chatgpt~\cite{paper71}
\item Does ChatGPT resemble humans in language use?~\cite{cai2023does}
\item A comprehensive capability analysis of gpt-3 and gpt-3.5 series models~\cite{paper73}
\item A comprehensive evaluation of ChatGPT's zero-shot Text-to-SQL capability~\cite{paper74}
\item Is ChatGPT a good sentiment analyzer? A preliminary study~\cite{paper75}
\item A preliminary evaluation of chatgpt for zero-shot dialogue understanding~\cite{paper76}
\item Zero-shot Temporal Relation Extraction with ChatGPT~\cite{paper77}
\item Can chatgpt reproduce human-generated labels? a study of social computing tasks~\cite{paper78}
\item Chatgraph: Interpretable text classification by converting chatgpt knowledge to graphs~\cite{paper79}
\item Uncovering the Potential of ChatGPT for Discourse Analysis in Dialogue: An Empirical Study~\cite{paper80}
\item Evaluating ChatGPT's Performance for Multilingual and Emoji-based Hate Speech Detection~\cite{paper81}
\item Sentiment Analysis in the Era of Large Language Models: A Reality Check~\cite{paper82}
\item ChatGPT for Suicide Risk Assessment on Social Media: Quantitative Evaluation of Model Performance, Potentials and Limitations~\cite{paper83}
\item Metacognitive Prompting Improves Understanding in Large Language Models~\cite{paper84}
\item Exploring ai ethics of chatgpt: A diagnostic analysis~\cite{paper85}
\item Is chatgpt better than human annotators? potential and limitations of chatgpt in explaining implicit hate speech~\cite{paper86}
\item Investigating Chain-of-thought with ChatGPT for Stance Detection on Social Media~\cite{paper87}
\item The Self-Perception and Political Biases of ChatGPT~\cite{paper88}
\item Not All Languages Are Created Equal in LLMs: Improving Multilingual Capability by Cross-Lingual-Thought Prompting~\cite{paper89}
\item BAD: BiAs Detection for Large Language Models in the context of candidate screening~\cite{paper90}
\item DECODINGTRUST: A Comprehensive Assessment of Trustworthiness in GPT Models~\cite{paper91}
\item On Large Language Models' Selection Bias in Multi-Choice Questions~\cite{paper92}
\item Exploring the Limits of ChatGPT for Query or Aspect-based Text Summarization~\cite{paper93}
\item ChatGPT as a Factual Inconsistency Evaluator for Text Summarization~\cite{paper94}
\item Uncovering ChatGPT's Capabilities in Recommender Systems~\cite{paper95}
\item HaluEval: A Large-Scale Hallucination Evaluation Benchmark for Large Language Models~\cite{paper96}
\item RecurrentGPT: Interactive Generation of (Arbitrarily) Long Text~\cite{paper97}
\item PokemonChat: Auditing ChatGPT for Pokémon Universe Knowledge~\cite{paper98}
\item Hybrid Long Document Summarization using C2F-FAR and ChatGPT: A Practical Study~\cite{paper99}
\item Generative Job Recommendations with Large Language Model~\cite{paper100}
\item Assessing the Ability of ChatGPT to Screen Articles for Systematic Reviews~\cite{paper101}
\item L-Eval: Instituting Standardized Evaluation for Long Context Language Models~\cite{paper102}
\item LLM-Rec: Personalized Recommendation via Prompting Large Language Models~\cite{paper103}
\item LongBench: A Bilingual, Multitask Benchmark for Long Context Understanding~\cite{paper104}
\item Can Large Language Models Understand Real-World Complex Instructions~\cite{paper105}
\item Mind meets machine: Unravelling GPT-4's cognitive psychology~\cite{paper106}
\item Capabilities of GPT-4 on Medical Challenge Problems~\cite{paper107}
\item GPT is becoming a Turing machine: Here are some ways to program it~\cite{paper108}
\item ChatGPT is a Knowledgeable but Inexperienced Solver: An Investigation of Commonsense Problem in Large Language Models~\cite{paper109}
\item Humans in Humans Out: On GPT Converging Toward Common Sense in both Success and Failure~\cite{paper110}
\item Generative Models as a Complex Systems Science: How can we make sense of large language model behavior?~\cite{paper111}
\item How well do Large Language Models perform in Arithmetic tasks?~\cite{paper112}
\item Uncertainty in Natural Language Generation: From Theory to Applications~\cite{paper113}
\item ChatGPT-Crawler: Find out if ChatGPT really knows what it's talking about~\cite{paper114}
\item How is ChatGPT's behavior changing over time?~\cite{chen2023chatgpt}
\item ChatABL: Abductive Learning via Natural Language Interaction with ChatGPT~\cite{paper116}
\item Look Before You Leap: An Exploratory Study of Uncertainty Measurement for Large Language Models~\cite{paper117}
\item StructGPT: A General Framework for Large Language Model to Reason over Structured Data~\cite{paper118}
\item Chain-of-Symbol Prompting Elicits Planning in Large Langauge Models~\cite{paper119}
\item Tree of Thoughts: Deliberate Problem Solving with Large Language Models~\cite{paper120}
\item ChatLog: Recording and Analyzing ChatGPT Across Time~\cite{paper121}
\item Chain of Knowledge: A Framework for Grounding Large Language Models with Structured Knowledge Bases~\cite{paper122}
\item ChatHaruhi: Reviving Anime Character in Reality via Large Language Model.~\cite{paper123}
\item Adaptive Chameleon or Stubborn Sloth: Unraveling the Behavior of Large Language Models in Knowledge Conflicts~\cite{paper124}
\item GPT-3.5 vs GPT-4: Evaluating ChatGPT's Reasoning Performance in Zero-shot Learning~\cite{paper125}
\item LogiCoT: Logical Chain-of-Thought Instruction-Tuning Data Collection with GPT-4~\cite{paper126}
\item Enabling Large Language Models to Generate Text with Citations~\cite{paper127}
\item Why Does ChatGPT Fall Short in Providing Truthful Answers?~\cite{paper128}
\item Are Large Language Models Really Good Logical Reasoners? A Comprehensive Evaluation From Deductive, Inductive and Abductive Views~\cite{paper129}
\item Investigating the Factual Knowledge Boundary of Large Language Models with Retrieval Augmentation~\cite{paper130}
\item SciBench: Evaluating College-Level Scientific Problem-Solving Abilities of Large Language Models~\cite{paper131}
\item Think-on-Graph: Deep and Responsible Reasoning of Large Language Model with Knowledge Graph~\cite{paper132}
\item Skills-in-Context Prompting: Unlocking Compositionality in Large Language Models~\cite{paper133}
\item Large Language Models Sensitivity to The Order of Options in Multiple-Choice Questions~\cite{paper134}
\item Large Language Models on the Chessboard: A Study on ChatGPT's Formal Language Comprehension and Complex Reasoning Skills~\cite{paper135}
\item Evaluating Large Language Models on Graphs: Performance Insights and Comparative Analysis~\cite{paper136}
\item Exploring New Frontiers in Agricultural NLP: Investigating the Potential of Large Language Models for Food Applications~\cite{paper137}
\item MINT: Evaluating LLMs in Multi-turn Interaction with Tools and Language Feedback~\cite{paper138}
\item ChatGPT for Robotics: Design Principles and Model Abilities~\cite{paper139}
\item Error Analysis Prompting Enables Human-Like Translation Evaluation in Large Language Models: A Case Study on ChatGPT~\cite{paper140}
\item Towards Making the Most of ChatGPT for Machine Translation~\cite{paper141}
\item Linguistically Informed ChatGPT Prompts to Enhance Japanese-Chinese Machine Translation: A Case Study on Attributive Clauses~\cite{paper142}
\item How to Design Translation Prompts for ChatGPT: An Empirical Study~\cite{paper143}
\item Is Your Code Generated by ChatGPT Really Correct? Rigorous Evaluation of Large Language Models for Code Generation~\cite{paper144}
\item Evaluating ChatGPT's Information Extraction Capabilities: An Assessment of Performance, Explainability, Calibration, and Faithfulness~\cite{paper145}
\item Can ChatGPT Assess Human Personalities? A General Evaluation Framework~\cite{paper146}
\item Is ChatGPT Equipped with Emotional Dialogue Capabilities?~\cite{paper147}
\item AugGPT: Leveraging ChatGPT for Text Data
Augmentation~\cite{paper148}
\item Evaluating GPT-4 and ChatGPT on Japanese Medical Licensing Examinations~\cite{paper149}
\item To ChatGPT, or not to ChatGPT: That is the question!~\cite{paper150}
\item In ChatGPT We Trust? Measuring and Characterizing the Reliability of ChatGPT~\cite{paper151}
\item Analyzing ChatGPT's Aptitude in an Introductory Computer Engineering Course~\cite{paper152}
\item Linguistic ambiguity analysis in ChatGPT~\cite{paper153}
\item Using ChatGPT for Entity Matching~\cite{paper154}
\item MEGA: Multilingual Evaluation of Generative AII~\cite{paper155}
\item Evaluation of ChatGPT on Biomedical Tasks: A Zero-Shot Comparison with Fine-Tuned Generative Transformers~\cite{paper156}
\item Zero-shot Clinical Entity Recognition using ChatGPT~\cite{paper157}
\item Human-like Summarization Evaluation with ChatGPT~\cite{paper158}
\item "HOT" ChatGPT: The promise of ChatGPT in detecting and discriminating hateful, offensive, and toxic comments on social media~\cite{paper159}
\item Large language models effectively leverage document-level context for literary translation, but critical errors persist~\cite{paper160}
\item BayLing: Bridging Cross-lingual Alignment and Instruction Following through Interactive Translation for Large Language Models~\cite{paper161}
\item Neural Machine Translation Data Generation and Augmentation using ChatGPT~\cite{paper162}
\item ChatGPT MT: Competitive for High- (but not Low-) Resource Languages~\cite{paper163}
\item How would Stance Detection Techniques Evolve after the Launch of ChatGPT?~\cite{zhang2022would}
\item BHASA: A Holistic Southeast Asian Linguistic and Cultural Evaluation Suite for Large Language Models~\cite{paper165}
\item Zero-shot Approach to Overcome Perturbation Sensitivity of Prompts~\cite{paper166}
\item UZH\_CLyp at SemEval-2023 Task 9: Head-First Fine-Tuning and ChatGPT Data Generation for Cross-Lingual Learning in Tweet Intimacy Prediction~\cite{paper167}
\item Exploring the Feasibility of ChatGPT for Event Extraction~\cite{paper168}
\item Does Synthetic Data Generation of LLMs Help Clinical Text Mining?~\cite{paper169}
\item ICL-D3IE: In-Context Learning with Diverse Demonstrations Updating for Document Information Extraction~\cite{paper170}
\item ChatGPT Prompt Patterns for Improving Code Quality, Refactoring, Requirements Elicitation, and Software Design~\cite{paper171}
\item SelfCheckGPT: Zero-Resource Black-Box Hallucination Detection for Generative Large Language Models~\cite{paper172}
\item Translating Radiology Reports into Plain Language using ChatGPT and GPT-4 with Prompt Learning: Promising Results, Limitations, and Potential~\cite{paper173}
\item An Empirical Study of Pre-trained Language Models in Simple Knowledge Graph Question Answering~\cite{paper174}
\item DeID-GPT: Zero-shot Medical Text De-Identification by GPT-4~\cite{paper175}
\item MM-REACT: Prompting ChatGPT for Multimodal Reasoning and Action~\cite{paper176}
\item Is ChatGPT A Good Keyphrase Generator? A Preliminary Study~\cite{paper177}
\item Beyond Black Box AI-Generated Plagiarism Detection: From Sentence to Document Level~\cite{paper178}
\item Comparing Abstractive Summaries Generated by ChatGPT to Real Summaries Through Blinded Reviewers and Text Classification Algorithms~\cite{paper179}
\item MGTBench: Benchmarking Machine-Generated Text Detection~\cite{paper180}
\item Neural Theory-of-Mind? On the Limits of Social Intelligence in Large LMs~\cite{paper181}
\item What would Harry say? Building Dialogue Agents for Characters in a Story~\cite{paper182}
\item Reliable Natural Language Understanding with Large Language Models and Answer Set Programming~\cite{paper183}
\item ByGPT5: End-to-End Style-conditioned Poetry Generation with Token-free Language Models~\cite{paper184}
\item Transformers Go for the LOLs: Generating (Humourous) Titles from Scientific Abstracts End-to-End~\cite{paper185}
\item Modeling Label Semantics Improves Activity Recognition~\cite{paper186}
\item An Analysis of the Automatic Bug Fixing Performance of ChatGPT~\cite{paper187}
\item Chat2VIS: Generating Data Visualisations via Natural Language using ChatGPT, Codex and GPT-3 Large Language Models~\cite{paper188}
\item ChatGPT versus Traditional Question Answering for Knowledge Graphs: Current Status and Future Directions Towards Knowledge Graph Chatbots~\cite{paper189}
\item ChatCAD: Interactive Computer-Aided Diagnosis on Medical Image using Large Language Models~\cite{paper190}
\item Guiding Large Language Mdels via Directional Stimulus Prompting~\cite{paper191}
\item Utilizing ChatGPT Generated Data to Retrieve Depression Symptoms from Social Media~\cite{paper192}
\item Check Your Facts and Try Again: Improving Large Language Models with External Knowledge and Automated Feedback~\cite{paper193}
\item ChatGPT for Zero-shot Dialogue State Tracking: A Solution or an Opportunity?~\cite{paper194}
\item ChatGPT vs Human-authored Text: Insights into Controllable Text Summarization and Sentence Style Transfer~\cite{paper195}
\item Not The End of Story: An Evaluation of ChatGPT-Driven Vulnerability Description Mappings~\cite{paper196}
\item ChatGPT is not a good indigenous translator~\cite{paper197}
\item You’ve Got a Friend in ... a Language Model? A Comparison of Explanations of Multiple-Choice Items of Reading Comprehension between ChatGPT and Humans~\cite{paper198}
\item Language-Agnostic Transformers and Assessing ChatGPT-Based Query Rewriting for Multilingual Document-Grounded QA~\cite{paper199}
\item HW-TSC at SemEval-2023 Task 7: Exploring the Natural Language Inference Capabilities of ChatGPT and Pre-trained Language Model for Clinical Trial~\cite{paper200}
\item Can ChatGPT Understand Causal Language in Science Claims?~\cite{paper201}
\item ChatGPT is fun, but it is not funny! Humor is still challenging Large Language Models~\cite{paper202}
\item Assessing Cross-Cultural Alignment between ChatGPT and Human Societies: An Empirical Study~\cite{paper203}
\item Evaluating Reading Comprehension Exercises Generated by LLMs: A Showcase of ChatGPT in Education Applications~\cite{paper204}
\item ChatGPT vs. Crowdsourcing vs. Experts: Annotating Open-Domain Conversations with Speech Functions~\cite{paper205}
\item Leveraging Large Language Models for Automated Dialogue Analysis~\cite{paper206}
\item Breaking the Bank with ChatGPT: Few-Shot Text Classification for Finance~\cite{paper207}
\item Is ChatGPT a Good Teacher Coach? Measuring Zero-Shot Performance For Scoring and Providing Actionable Insights on Classroom Instruction~\cite{paper208}
\item Credible Without Credit: Domain Experts Assess Generative Language Models~\cite{paper209}
\item SUT at SemEval-2023 Task 1: Prompt Generation for Visual Word Sense Disambiguation~\cite{paper210}
\item How Well Do Large Language Models Perform on Faux Pas Tests?~\cite{paper211}
\item Zero-Shot Information Extraction for Clinical Meta-Analysis using Large Language Models~\cite{paper212}
\item Can Large Language Models Be an Alternative to Human Evaluation?~\cite{paper213}
\item RL4F: Generating Natural Language Feedback with Reinforcement Learning for Repairing Model Outputs~\cite{paper214}
\item Toward Human-Like Evaluation for Natural Language Generation with Error Analysis~\cite{paper215}
\item Multi-Level Knowledge Distillation for Out-of-Distribution Detection in Text~\cite{paper216}
\item MolXPT: Wrapping Molecules with Text for Generative Pre-training~\cite{paper217}
\item MUX-PLMs: Pre-training Language Models with Data Multiplexing~\cite{paper218}
\item Is GPT-3 a Good Data Annotator?~\cite{paper219}
\item Language Generation Models Can Cause Harm: So What Can We Do About It? An Actionable Survey~\cite{paper220}
\item Detoxifying Online Discourse: A Guided Response Generation Approach for Reducing Toxicity in User-Generated Text~\cite{paper221}
\item Faithful Question Answering with Monte-Carlo Planning~\cite{paper222}
\item Nut-cracking Sledgehammers: Prioritizing Target Language Data over Bigger Language Models for Cross-Lingual Metaphor Detection~\cite{paper223}
\item Generating Faithful Text From a Knowledge Graph with Noisy Reference Text~\cite{paper224}
\item Empowering Conversational Agents using Semantic In-Context Learning~\cite{paper225}
\item Can Large Language Models Safely Address Patient Questions Following Cataract Surgery?~\cite{paper226}
\item Towards Benchmarking and Improving the Temporal Reasoning Capability of Large Language Models~\cite{paper227}
\item Generative Pretrained Transformers for Emotion Detection in a Code-Switching Setting~\cite{paper228}
\item On the Underspecification of Situations in Open-domain Conversational Datasets~\cite{paper229}
\item Understanding Factual Errors in Summarization: Errors, Summarizers, Datasets, Error Detectors~\cite{paper230}
\item Multilingual Language Models are not Multicultural: A Case Study in Emotion~\cite{paper231}
\item Good Data, Large Data, or No Data? Comparing Three Approaches in Developing Research Aspect Classifiers for Biomedical Papers~\cite{paper232}
\item IDOL: Indicator-oriented Logic Pre-training for Logical Reasoning~\cite{paper233}
\item PrecogIIITH@WASSA2023: Emotion Detection for Urdu-English Code-mixed Text~\cite{paper234}
\item Do PLMs Know and Understand Ontological Knowledge?~\cite{paper235}
\item Evaluation of Question Generation Needs More References~\cite{paper236}
\item A System for Answering Simple Questions in Multiple Languages~\cite{paper237}
\item HIT-SCIR at WASSA 2023: Empathy and Emotion Analysis at the Utterance-Level and the Essay-Level~\cite{paper238}
\item Pre-trained Language Models Can be Fully Zero-Shot Learners~\cite{paper239}
\item Predicting the Quality of Revisions in Argumentative Writing~\cite{paper240}
\item Exploring Effectiveness of GPT-3 in Grammatical Error Correction: A Study on Performance and Controllability in Prompt-Based Methods~\cite{paper241}
\item When Truth Matters – Addressing Pragmatic Categories in Natural Language Inference (NLI) by Large Language Models (LLMs)~\cite{paper242}
\item Debiasing should be Good and Bad: Measuring the Consistency of Debiasing Techniques in Language Models~\cite{paper243}
\item GPoeT: a Language Model Trained for Rhyme Generation on Synthetic Data~\cite{paper244}
\item Examining Bias in Opinion Summarisation Through the Perspective of Opinion Diversity~\cite{paper245}
\item Unsupervised Summarization Re-ranking~\cite{paper246}
\item Improving Dutch Vaccine Hesitancy Monitoring via Multi-Label Data Augmentation with GPT-3.5~\cite{paper247}
\item What Makes a Good Counter-Stereotype? Evaluating Strategies for Automated Responses to Stereotypical Text~\cite{paper248}
\item What Makes Good Counterspeech? A Comparison of Generation Approaches and Evaluation Metrics~\cite{paper249}
\item DAMO-NLP at SemEval-2023 Task 2: A Unified Retrieval-augmented System for Multilingual Named Entity Recognition~\cite{paper250}
\item UMASS\_BioNLP at MEDIQA-Chat 2023: Can LLMs generate high-quality synthetic note-oriented doctor-patient conversations?~\cite{paper251}
\item Frontier Review of Multimodal AI~\cite{paper252}
\item Is ChatGPT a Highly Fluent Grammatical Error Correction System? A Comprehensive Evaluation~\cite{paper253}
\item DialogStudio: Towards Richest and Most Diverse Unified Dataset Collection for Conversational AI~\cite{paper254}
\end{itemize} 
 

==> review2.tex <==
\nociteRev{paper0}
\nociteRev{golchin2023time}
\nociteRev{gururangan-etal-2020-dont}
\nociteRev{paper3}
\nociteRev{paper4}
\nociteRev{paper5}
\nociteRev{paper6}
\nociteRev{paper7}
\nociteRev{ippolito-etal-2023-preventing}
\nociteRev{paper9}
\nociteRev{paper10}
\nociteRev{paper11}
\nociteRev{paper12}
\nociteRev{shi2023dont}
\nociteRev{paper14}
\nociteRev{paper15}
\nociteRev{paper16}
\nociteRev{paper17}
\nociteRev{paper18}
\nociteRev{paper19}
\nociteRev{chatpgt-jack-trades-master-none}
\nociteRev{paper21}
\nociteRev{paper22}
\nociteRev{paper23}
\nociteRev{paper24}
\nociteRev{paper25}
\nociteRev{paper26}
\nociteRev{paper27}
\nociteRev{paper28}
\nociteRev{paper29}
\nociteRev{paper30}
\nociteRev{paper31}
\nociteRev{paper32}
\nociteRev{paper33}
\nociteRev{paper34}
\nociteRev{paper35}
\nociteRev{paper36}
\nociteRev{paper37}
\nociteRev{paper38}
\nociteRev{paper39}
\nociteRev{paper40}
\nociteRev{paper41}
\nociteRev{paper42}
\nociteRev{paper43}
\nociteRev{paper44}
\nociteRev{paper45}
\nociteRev{paper46}
\nociteRev{paper47}
\nociteRev{paper48}
\nociteRev{paper49}
\nociteRev{paper50}
\nociteRev{paper51}
\nociteRev{paper52}
\nociteRev{paper53}
\nociteRev{paper54}
\nociteRev{paper55}
\nociteRev{paper56}
\nociteRev{paper57}
\nociteRev{paper58}
\nociteRev{paper59}
\nociteRev{paper60}
\nociteRev{paper61}
\nociteRev{paper62}
\nociteRev{paper63}
\nociteRev{paper64}
\nociteRev{paper65}
\nociteRev{paper66}
\nociteRev{paper67}
\nociteRev{paper68}
\nociteRev{paper69}
\nociteRev{paper70}
\nociteRev{paper71}
\nociteRev{cai2023does}
\nociteRev{paper73}
\nociteRev{paper74}
\nociteRev{paper75}
\nociteRev{paper76}
\nociteRev{paper77}
\nociteRev{paper78}
\nociteRev{paper79}
\nociteRev{paper80}
\nociteRev{paper81}
\nociteRev{paper82}
\nociteRev{paper83}
\nociteRev{paper84}
\nociteRev{paper85}
\nociteRev{paper86}
\nociteRev{paper87}
\nociteRev{paper88}
\nociteRev{paper89}
\nociteRev{paper90}
\nociteRev{paper91}
\nociteRev{paper92}
\nociteRev{paper93}
\nociteRev{paper94}
\nociteRev{paper95}
\nociteRev{paper96}
\nociteRev{paper97}
\nociteRev{paper98}
\nociteRev{paper99}
\nociteRev{paper100}
\nociteRev{paper101}
\nociteRev{paper102}
\nociteRev{paper103}
\nociteRev{paper104}
\nociteRev{paper105}
\nociteRev{paper106}
\nociteRev{paper107}
\nociteRev{paper108}
\nociteRev{paper109}
\nociteRev{paper110}
\nociteRev{paper111}
\nociteRev{paper112}
\nociteRev{paper113}
\nociteRev{paper114}
\nociteRev{chen2023chatgpt}
\nociteRev{paper116}
\nociteRev{paper117}
\nociteRev{paper118}
\nociteRev{paper119}
\nociteRev{paper120}
\nociteRev{paper121}
\nociteRev{paper122}
\nociteRev{paper123}
\nociteRev{paper124}
\nociteRev{paper125}
\nociteRev{paper126}
\nociteRev{paper127}
\nociteRev{paper128}
\nociteRev{paper129}
\nociteRev{paper130}
\nociteRev{paper131}
\nociteRev{paper132}
\nociteRev{paper133}
\nociteRev{paper134}
\nociteRev{paper135}
\nociteRev{paper136}
\nociteRev{paper137}
\nociteRev{paper138}
\nociteRev{paper139}
\nociteRev{paper140}
\nociteRev{paper141}
\nociteRev{paper142}
\nociteRev{paper143}
\nociteRev{paper144}
\nociteRev{paper145}
\nociteRev{paper146}
\nociteRev{paper147}
\nociteRev{paper148}
\nociteRev{paper149}
\nociteRev{paper150}
\nociteRev{paper151}
\nociteRev{paper152}
\nociteRev{paper153}
\nociteRev{paper154}
\nociteRev{paper155}
\nociteRev{paper156}
\nociteRev{paper157}
\nociteRev{paper158}
\nociteRev{paper159}
\nociteRev{paper160}
\nociteRev{paper161}
\nociteRev{paper162}
\nociteRev{paper163}
\nociteRev{zhang2022would}
\nociteRev{paper165}
\nociteRev{paper166}
\nociteRev{paper167}
\nociteRev{paper168}
\nociteRev{paper169}
\nociteRev{paper170}
\nociteRev{paper171}
\nociteRev{paper172}
\nociteRev{paper173}
\nociteRev{paper174}
\nociteRev{paper175}
\nociteRev{paper176}
\nociteRev{paper177}
\nociteRev{paper178}
\nociteRev{paper179}
\nociteRev{paper180}
\nociteRev{paper181}
\nociteRev{paper182}
\nociteRev{paper183}
\nociteRev{paper184}
\nociteRev{paper185}
\nociteRev{paper186}
\nociteRev{paper187}
\nociteRev{paper188}
\nociteRev{paper189}
\nociteRev{paper190}
\nociteRev{paper191}
\nociteRev{paper192}
\nociteRev{paper193}
\nociteRev{paper194}
\nociteRev{paper195}
\nociteRev{paper196}
\nociteRev{paper197}
\nociteRev{paper198}
\nociteRev{paper199}
\nociteRev{paper200}
\nociteRev{paper201}
\nociteRev{paper202}
\nociteRev{paper203}
\nociteRev{paper204}
\nociteRev{paper205}
\nociteRev{paper206}
\nociteRev{paper207}
\nociteRev{paper208}
\nociteRev{paper209}
\nociteRev{paper210}
\nociteRev{paper211}
\nociteRev{paper212}
\nociteRev{paper213}
\nociteRev{paper214}
\nociteRev{paper215}
\nociteRev{paper216}
\nociteRev{paper217}
\nociteRev{paper218}
\nociteRev{paper219}
\nociteRev{paper220}
\nociteRev{paper221}
\nociteRev{paper222}
\nociteRev{paper223}
\nociteRev{paper224}
\nociteRev{paper225}
\nociteRev{paper226}
\nociteRev{paper227}
\nociteRev{paper228}
\nociteRev{paper229}
\nociteRev{paper230}
\nociteRev{paper231}
\nociteRev{paper232}
\nociteRev{paper233}
\nociteRev{paper234}
\nociteRev{paper235}
\nociteRev{paper236}
\nociteRev{paper237}
\nociteRev{paper238}
\nociteRev{paper239}
\nociteRev{paper240}
\nociteRev{paper241}
\nociteRev{paper242}
\nociteRev{paper243}
\nociteRev{paper244}
\nociteRev{paper245}
\nociteRev{paper246}
\nociteRev{paper247}
\nociteRev{paper248}
\nociteRev{paper249}
\nociteRev{paper250}
\nociteRev{paper251}
\nociteRev{paper252}
\nociteRev{paper253}
\nociteRev{paper254}
 
